Private Information Acquisition and Preemption: a Strategic Wald Problem

This paper studies a dynamic information acquisition model with payoff externalities. Two players can acquire costly information about an unknown state before taking a safe or risky action. Both information and the action taken are private. The first player to take the risky action has an advantage but whether the risky action is profitable depends on the state. The players face the tradeoff between being first and being right. In equilibrium, for different priors, there exist three kinds of randomisation: when the players are pessimistic, they enter the competition randomly; when the players are less pessimistic, they acquire information and then randomly stop; when the players are relatively optimistic, they randomly take an action without acquiring information.

==> best_responses.tex <==
\subsection{Formulation of the player's problem}
\label{subsec:bestresponses}




This section formulates one player's problem given opponent's strategies.
Given player $j$'s strategy $\gamma^{j}$, player $i$'s best-reply problem is to choose a time $T^{i}$ with value function 
$
\hat{V}^{i,\gamma^{j}}:\mathbb{R}_{+}\rightarrow \mathbb{R}
$ 
such that
\begin{align}
\hat{V}^{i,\gamma^{j}}\left(0\right)
&:=
\max_{T^{i}}\intop_{0}^{T^{i}}\pi_{t}\left[p_{t}^{i}a\mathbb{E}^{\gamma^{j}}\left[u_{H}^{R}\mid H,t\right]-c\right]dt+\pi_{T^{i}}U^{i,\gamma^{j}}\left(T^{i}\right)
\\
&\text{s.t. }\frac{dp_{t}^{i}}{dt}=(b-a)p_{t}^{i}(1-p_{t}^{i}),
\nonumber
\end{align}
where 
$
\mathbb{E}^{\gamma^{j}}\left[u_{H}^{R}\mid H,t\right]
$
and 
$
U^{i,\gamma^{j}}\left(T^{i}\right)
$
is defined in \Cref{sub:strategiesandequilibrium}.
The Hamilton-Jacobi-Bellman (HJB) equation for player $i$'s problem is the following differential equation in 
$
V^{i,\gamma^{j}}:\mathbb{R}_{+}\rightarrow \mathbb{R},
$
where
\begin{align}
\label{eq:hjbequation}
\max
\left\{
\overbrace{
p_{t}^{i}a\left[\mathbb{E}^{\gamma^{j}}\left[u_{H}^{R}\mid H,t\right]
-
V^{i,\gamma^{j}}\left(t\right)\right]
+
\left(1-p_{t}^{i}\right)b\left[-V^{i,\gamma^{j}}\left(t\right)\right]
}
^{\text{A}}
+
\overbrace{
\frac{dV^{i,\gamma^{j}}\left(t\right)}{dt}
}
^
{\text{B}}
-c,\right.
\nonumber
\\
\left.
U^{i,\gamma^{j}}\left(t\right)
-
V^{i,\gamma^{j}}\left(t\right)
\right\}  
& =0
.
\end{align}
The interpretation of (\ref{eq:hjbequation}) is that at time $t$, player $i$ chooses between to continue acquiring information or stopping. 
She acquires information if the marginal gain is greater than the marginal cost.
Otherwise, she stops and gets the payoff 
$
U^{i,\gamma^{j}}\left(t\right)
$.
The marginal gain consists of the expected gain from receiving the revealing signal (labelled as A in (\ref{eq:hjbequation})) plus the rate of change of the value (labelled as B in (\ref{eq:hjbequation})).














Given opponent's strategy 
$
\gamma^{j}
$, 
if the player's problem is well-behaved, then, the value function 
$
V^{i,\gamma^{j}}\left(t\right)
$
is a classical solution to the HJB equation (\ref{eq:hjbequation}).
The player's best response can then be characterised correspondingly.
However, in our problem, (\ref{eq:hjbequation}) is not well-behaved because given the opponent's strategy 
$
\gamma^{j}
$,
$
U^{i,\gamma^{j}}\left(t\right)
$
has a kink and may not be continuous.
The 














 


%This section shows that player $i$'s best response to player $j$'s mixed strategy consists of random stopping.
%This suggests the use of mixed strategies in equilibrium.
%Next section introduces the strategies that appear in equilibrium.


















%When prior is in the intermediary range, player $i$'s best response is to acquire information at time $0$.
%When the belief drifts up, player $i$ acquires information at each time $t$ if the marginal gain is greater than the marginal cost.
%Given player $j$'s mixed strategy, the marginal gain and the marginal cost can be the same for a period of time.
%When this happens, player $i$ randomises between immediate stopping and acquiring information for $dt$ longer.

==> equilibrium_analysis_subsections/multiple_equilibria.tex <==
\subsection{Multiple equilibria}
\label{subsec:multipleequilibria}



There are multiple equilibria when the prior is in the intermediate range.


\begin{lemma}
\label{lemma:multipleequilibria} 
When $c$ is sufficiently small, there exist multiple equilibria if $\underline{p}<p_{0}<p^{M}$.
\end{lemma}




When
$p^{*}\leq p_{0}<\tilde{p}$, there exists an equilibrium where both players use the Random Stopping Strategy.
The time at which the players start randomising is not unique and this leads to multiple equilibria.
To get the intuition, suppose player $j$ uses the Random Stopping Strategy which starts randomising at some time $\hat{T}>0$.
Then, to have both players using this strategy as an equilibrium, before time $\hat{T}$, player $i$ strictly prefers to acquire information given that the opponent acquires information.
After time $\hat{T}$, player $i$ prefers to randomise instead of taking $S$.
As a result, the latest time at which the player starts randomising is the first time instant at which the marginal cost of acquiring information equals the marginal benefit given that the opponent acquires information.
The earliest time at which the player is willing to start randomising satisfies the condition that given the opponent starts randomising, the player prefers to randomise instead of taking $S$.
These two time points do not coincide and hence pin down an interval of time at which the randomisation could start.
The intuition behind the multiplicity is the strategic complementarity of information.
Information is a strategic complement at time $t<\hat{T}$ because when the opponent is still acquiring information, the value of information is relatively high.
The player hence is also willing to acquire more information.
If the opponent starts randomising, then, the value associated with acquiring information becomes lower.
The player then matches the time at which the opponent starts randomising.
This strategic complementarity also explains the existence of multiple equilibria when 
$
p_{0} 
\in
\left[
p^{L},p^{M}
\right)
$.
For this range of priors, according to \Cref{thm:mainresult}, 
there exist both kinds of equilibria where the players use the Random Stopping Strategy and where the players use the Immediate Mix Strategy.
In other words, there simultaneously exist the equilibria where the players acquire information and where the players do not acquire information.



